Horizon Instability of the Extremal BTZ Black Hole

We study real-time propagation of a massive scalar field on the extremal BTZ black hole spacetime, focusing on the Aretakis instability of the event horizon. We obtain a simple time-domain expression for the $\textrm{AdS}_3$ retarded Green function with Dirichlet boundary conditions and construct the corresponding time-domain BTZ retarded Green function using the method of images. The field decays at different rates on and off the horizon, indicating that transverse derivatives grow with time on the horizon (Aretakis instability). We solve the null geodesic equation in full generality and show that the instability is associated with a class of null geodesics that orbit near the event horizon arbitrarily many times before falling in. In an appendix we also treat the problem in the frequency domain, finding consistency between the methods.

==> nearextremal.tex <==
\section{Near Extremal BTZ}\label{sec:nearModes}
We now consider the quasinormal mode ringing of massive mode-perturbations to the near-extremal BTZ black hole.

The sub-extremal BTZ metric is 
\begin{equation}\label{holla for tha dolla}
ds^2 = - \frac{ (R^2 - R_-^2)(R^2 - R_+^2) }{
R^2} dT^2  
+ \frac{ R^2 }{ ( R^2-R_-^2)(R^2-R_+^2) } dR^2 + R^2 \left(dX - \frac{R_+ R_-}{R^2} dT  \right)^2.
\end{equation}
The solution has an inner and outer horizon, $R_-$ and $R_+$, with associated temperatures 
\begin{equation}
    T_\pm = \frac{R_+^2-R_-^2}{2 \pi R_\pm}
\end{equation}
and angular velocities
\begin{equation}
    \Omega_\pm=\frac{R_\mp}{R_\pm}.
\end{equation}
The inner and outer horizon radii $R_\pm$ are related to the mass $M$ and angular momentum $J$  of the black hole
by
\begin{equation}
    R_\pm = \frac{M}{2} \left(1\pm \sqrt{1- \frac{J^2}{M^2}}  \right)^{1/2}.
\end{equation}
%(the conserved charges associated with the asymptotic Killing vectors $\pd_T$ and $\pd_\Phi$ at asymptotic Anti-de-Sitter spaces as defined by Abbot and Deser \cite{Abbott:1981ff}).
At the extremal limit, $M=J \implies R_+ = R_- \equiv R_H = M/2$. 

To avoid tracking factors of $\pi$ we also define
\begin{equation}
%\k_\pm=2\pi R_\pm T_\pm.
\k_\pm=2\pi T_\pm.
\end{equation}

As before, we seek late-time, fixed-frequency solutions of the massive wave equation
\begin{equation}
(\Box - \mu^2)\psi=0
\end{equation}
by mode decomposition and variable separation. Following \cite{Ichinose:1994rg}, we separate variables by introducing the coordinate 
\begin{equation}\label{eq:r def}
\x=R^2-R_+^2, %\qquad \eta=X-\Omega_+ T
\end{equation}
For conveniance, we also introduce the barred quantities
\begin{equation}\label{eq:barred defs}
\bx = \frac{r}{R_+^2-R_-^2}, \qquad \bar \omega_\pm = \frac{(\omega-m\Omega_\pm)}{2\k_\pm}.
%= \frac{\omega}{4\pi T_H}.
%\frac{R_+(\omega-m\Omega_H)}{2\k} = \frac{\omega-m\Omega_H}{4\pi T_H}.
\end{equation}
A linearly independent set of radial solutions valid near infinity are 
\begin{equation}\label{eq:Rpm TBTZ}
R^{\rm \pm} 
=\bx^{-i\bar\omega_+}(1+\bx)^{i\bar\omega_+-h_\pm}{}_1F_1\left(h_\pm-i(\bar\omega_+-\bar\omega_-),h_\pm-i(\bar\omega_++\bar\omega_-);2h_\pm;\frac{1}{1+\bx}\right),
\end{equation}
where
\begin{equation}\label{eq:hpm def}
    h_\pm=\frac12 \pm\frac12 \sqrt{1+\mu^2}
\end{equation}
The boundary asymptotics are $R^\pm \sim \bx^{-h_\pm},\ \bx \to \infty$. 
We also require in the ingoing solution at the horizon
\begin{equation}\label{eq:Rin TBTZ}
R_{\rm in} =
\bx^{-i\bar\omega_+}\left(1+\bx\right)^{i\bar\omega_-}{}_2F_1\left(h_+-i(\bar\omega_+ +\bar\omega_-),h_--i(\bar\omega_++\bar\omega_-);1-2i\bar\omega_-;-\bx\right)
\end{equation}

The corresponding transfer function for the set of solutions $\{R_{\rm in},R^+\}$ is
\begin{equation}
g_m(\bx,\bx',\bar k) =  \frac{R_{\rm in}(\bx_<) R^+(\bx_>)}{\mathcal W},
\end{equation}
where the Wronskian is given by
\begin{align}\label{eq:W near}
 \mathcal W=
 (1-2h_+) \pi\csc(\pi(1-2h_+))
 \frac{\Gamma(1-2i\op)}{\Gamma(2h_-)\Gamma(h_+-i\op+i\om)\Gamma(h_+-i\op-i\om)}.
 %D_-
\end{align}
%$\mathcal W=\bx'(\bx'+1)\boldsymbol{W}[R_{\rm in},R_+]$ \PZ{check}.
%Using \href{https://dlmf.nist.gov/15.8}{DLMF 15.8.2} we express $R_{\rm in}$ in terms of $R_\pm$ as 
%\begin{equation}\label{eq:Rin(R_+,R_-)}
%R_{\rm in} = \pi\csc(\pi(2h_+-1))\Gamma(1-2 i\bk-2i\sm)(D_+ R_+ + D_-R_-),
%\end{equation}
%where
%\begin{equation}\label{eq:Dpm}
%D_\pm = \pm \frac{1}{\Gamma(2h_\pm)\Gamma(h_\mp-i\sm)\Gamma(h_\mp-2i\bk-i\sm)}.
%\end{equation}
The in solution satisfies the Dirichlet condition at infinity when $\mathcal W=0$. 
There exists two sets of quasinormal modes frequencies \cite{} for which  $\mathcal W$ vanishes 
\begin{equation}
\omega_n^{\pm}= \pm m - 2i(R_+ \mp R_-)(h_++n), \qquad n=0,1,2,\ldots.
\end{equation}
In the extremal limit $\omega_n^+$, the ``corotating'' frequency, becomes arbitrarily long-lived. We shall focus on these modes, as they are the relevant ones for the Aretakis instability. 

To determine the field resulting from the collective excitation of the long-lived quasinormal modes \eqref{eq:qnms}. For this we require the residues of the poles. 
%From Eqs.~\eqref{eq:Rin(R_+,R_-)} and \eqref{eq:Rpm TBTZ} we find that the Wronksian is given by
%\begin{equation}\label{eq:Wron Jeremy}
%\boldsymbol{W}[R_{\rm in},R_{+}]= \pi\csc(\pi(2h_+-1)) \Gamma(1-2i\bk-2i\sm)D_-W[R_-,R_+].
%\end{equation}
%Using \href{https://dlmf.nist.gov/15.10}{DLMF 15.10.7}, we find that 
%\begin{equation}
%\boldsymbol{W}[R_-,R_+]= %\frac{(1-2h_+)}{\bx'(1+\bx')}. %\bx^{2i\s}m
%\end{equation}
%\PZ{check}
For small $\kappa_\pm$, expanding $\mathcal W$ in an $\epsilon$-neighborhood of the poles gives
\begin{equation}
\mathcal W \approx \frac{\pi \csc(2\pi h_+)}{\Gamma(2h_-1)\Gamma(h_+-i\sm)} n! (-1)^n\Gamma(h_--n-i\sm)\epsilon
\end{equation}
to leading-order in $\epsilon$. Furthermore, at small-$\sigma$ the relevant radial functions are
\begin{align}
    R^+ &\approx
\end{align}
%Keep in mind that we have decomposed in the frequency $\omega$, so we need $\pd_\omega \mathcal W = R_+/(2\k)\pd_{\bar\omega }\mathcal W= R_+/(2\k)(-2i)\pd_{\epsilon}\mathcal W $.

\PZ{stopped here}
The usual definitions 
\begin{equation}
V=T+R_*, \qquad \Phi=X-\Omega_+T+\Phi_\sharp.
\end{equation}
For small $\kappa$,
\begin{align}\label{eq:rs ps}
R_* &\approx \frac{R_+}{2\k}\left(\log\left(
\frac{\bx}{1+\bx}\right)\right) + \frac{1}{4R_+}\log(\k) , \\ \Phi_\sharp &\approx\frac{R_+\Omega_H}{2 \k}\left(\log\left(
\frac{\bx}{1+\bx}\right)\right) - \frac{1}{2 r_+}\log(\k).
\end{align}
%A useful relation is 
%\begin{equation}
%e^{i\omega r_*-im\phi_\sharp}=\left(\frac{\bx}{1+\bx}\right)^{i\bk}\k^{i\sm}.
%\end{equation}
For a source point far from the horizon, we find the QNM contribution to the Green function $m$-modes reads  
\begin{align}
g^{\rm nf, QNM}_{m}(\bx,\bx';\delta \bar V)
=\frac{\bx{'}^{-h_+} 
\k^{1-h_++i\sm}}{2\pi r_+}  \frac{\Gamma(h_+-i\sm)}{\Gamma(2h_+)}
\sum_{n} e^{-(n+h_+)\delta\bar V}   
 \frac{  (-1)^n{}_2F_1(h_--i\sm,h_+-i\sm,h_--i\sm-n,-\bx)}{n!\Gamma(h_--i\sm-n)}  ,
\end{align}
where 
\begin{equation}
\delta \bar V= \k(V-V')/R_+
\end{equation}
The overtone sum has been performed already in previous work \cite{Gralla:2016sxp}. Using the result
\begin{align}
& \sum_n \frac{(-1)^ne^{-n\bar V}{}_2F_1(h_--i\sm,h_+-i\sm,h_--n-i\sm,-\bx)}{n!\Gamma(h_--n-i\sm)}
=\frac{\left(1-e^{-\bar V}\right)^{h_--i\sm-1}}{\Gamma(h_--i\sm)}\left(1+\bx(1-e^{-\bar V})\right)^{-h_++i\sm}
\end{align}
we find that
\begin{align}
g^{\rm nf, QNM}_{m} (\bx,\bx';\delta \bar V)
&=  \frac{\k^{h_-}}{2\pi\,\Gamma(2h_+)r_+}e^{-h_+\bar V} 
\left(1+\bx(1-e^{-\bar V})\right)^{-h_+}
\left(1-e^{-\bar V}\right)^{h_--1} \sum_m \frac{\Gamma(h_+-i\sm)}{\Gamma(h_--i\sm)} \mathcal Z^{i\sm} ,
\end{align}
where
\begin{equation}
\mathcal Z:= \k \left(1+\bx(1-e^{-\bar V})\right)\left(1-e^{-\bar V}\right).
\end{equation}
At large $m>0$, the absolute value of the summand diverges
\begin{equation}
\Bigg\vert  \frac{\Gamma(h_+-i\sm)}{\Gamma(h_--i\sm)} \Bigg\vert \sim m^{2h_+-1}, \qquad m \to \infty.
\end{equation}
\PZ{What to make of this???}

In the planar limit  summation goes over to integration and we can use Cauchy's theorem to 
resolve the integral by summing over the residues at $\sm=-i(n+h_+)$. The result is 
\begin{equation}
\int_{-\infty}^{\infty} \frac{\Gamma(h_+-i\sm)}{\Gamma(h_--i\sm)} \mathcal Z^{\sm}  d\sm = \frac{-2\pi\mathcal Z^{h_+}(1-\mathcal Z)^{-2h_+}}{\Gamma(1-2h_+)} - \text{arc.}
\end{equation}
The term $(1-\mathcal Z)$ is a non-self-similar  contribution to the QNM response at early-times.


%
%
%


\section{Arun's Derivation of Kirchhoff (saving for referenece; will not go in paper)}

Starting with 
\begin{equation}
    G_{\text{ret}} (x,x') (\Box' - m^2) \psi(x') = 0 \qquad \psi(x') (\Box' - m^2) G_{\text{ret}}(x,x') = \delta_{3} (x,x') \psi(x')
\end{equation}
Subtracting one from the other we obtain
\begin{equation}
    \nabla_{\alpha'}\left(\psi(x') \nabla^{\alpha'} G_{\text{ret}}(x,x') -G_{\text{ret}}(x,x') \nabla^{\alpha'} \psi(x') \right) = -\delta_3 (x,x') \psi(x').
\end{equation}
We can then use Stoke's theorem to integrate this in a closed volume $V$ giving us
\begin{equation}
    \oint_{\partial V}  \left(\psi(x') \nabla^{\alpha'} G_{\text{ret}}(x,x') -G_{\text{ret}}(x,x') \nabla^{\alpha'} \psi(x') \right) d\Sigma_{\alpha'} = \psi(x)
\end{equation}\AR{discrepancy using V for volume and ingoing time. Also discrepancy with using $\Sigma$ for surface and distance in AdS3}
where $\oint_{\partial V}$ denotes that the integral is performed on the boundary of the closed volume with the directed surface element denoted by $d\Sigma_{\alpha'}$.

We choose to use 3 surfaces $\Sigma_{1}$, $\Sigma_{2}$ and $\Sigma_{3}$ to enclose a closed volume in the spacetime. \AR{would be nice to have figures of these surfaces}
\begin{itemize}
    \item $\Sigma_{1}$ is a null surface defined by $\zeta^{1}(x^{\alpha}) = V - C_{1} =0$, a constant $V$ surface. This is a null surface since $g^{\alpha \beta} \zeta^{1}_{, \alpha} \zeta^{1}_{, \beta} = g^{VV} = 0$. We choose this surface to extend all the way from the boundary ($R \rightarrow \infty$) to inside the horizon ($R<R_{H}$). Here the coordinate $x$ is the parameter that takes you along the null geodesic.
    \item $\Sigma_{2}$ is a time-like surface on the boundary of the spacetime defined by $\zeta^{2}(x^{\alpha}) = R - c_{2} = 0$, a constant $x$ surface as $x \rightarrow \infty$ which is the boundary. This is a time-like surface since $g^{\alpha \beta} \zeta^{2}_{, \alpha} \zeta^{2}_{, \beta} = g^{RR} = \frac{R^2R_{H}^2}{R^2} >0$. We choose this surface to extend from the point where $\Sigma_{1}$ hits the boundary all the way to the late future where it will intersect with the third hypersurface. 
    \item $\Sigma_{3}$ is a space-like surface that closes the volume where it intersects with $\Sigma_{1}$ and $\Sigma_{2}$. It is chosen in such a way that on this surface, assuming there is no data specified on $\Sigma_{1}$ for $x<0$, the Green function on this hypersurface will be causally disconnected with any point in the interior of the volume created by these three hypersurfaces.
\end{itemize}
We impose Dirichlet reflecting conditions for the field on the surface $\Sigma_{2}$. This means that the field decays at a rate $\psi(R) \sim R^{-2h}$ as $R\rightarrow \infty$ on the boundary. Therefore the contribution to the integral by the surface $\Sigma_2$ is zero. By definition, the contribution to the closed integral from the surface $\Sigma_{3}$ is 0 since it is not in causal contact to any point in the exterior of the black hole. So the only contribution to the integral is by the surface $\Sigma_1$.

The surface element for the null surface of constant $V$ is 
\begin{equation}
    d\Sigma_{\alpha'}= \frac{R'}{R_{H}}dR' d \Phi' \{ 1,0,0\}
\end{equation}
resulting in the scalar field at any point in the exterior of the horizon being described by
